APPLE: An Evolution Code for Modeling Giant Planets

We introduce APPLE, a novel planetary evolution code designed specifically for the study of giant exoplanet and Jovian planet evolution in the era of Galileo, Juno, and Cassini. With APPLE, state-of-the-art equations of state for hydrogen, helium, ice, and rock are integrated with advanced features to treat ice/rock cores and metals in the gaseous envelope; models for helium rain and hydrogen/helium immiscibility; detailed atmosphere boundary tables that also provide self-consistent albedos and spectra; and options to address envelope metal gradients and stably-stratified regions. Our hope is that these purpose-built features of APPLE will help catalyze the development of the next generation of giant exoplanet and Jovian planet evolutionary models.

==> intro_old.tex <==
Jupiter and Saturn, two of the most fascinating planets in our Solar System, were formed about 4.56 billion years ago. They are known as the gas giants and are primarily composed of Hydrogen (H) and Helium (He), with traces of heavy elements such as methane, water, and ammonia. The combined mass of these planets accounts for over 92\% of the total mass of our Solar System. Despite their importance, the interiors of these planets remain enigmatic. They are ideal for studying materials under high pressures, such as the megabar (Mbar) pressure scales at temperatures of $10^4$ K, which is beyond the reach of terrestrial experiments. The processes that have shaped these planets over billions of years, and their evolution over time, have been studied for many years, yet much remains to be learned. By examining the chemical composition, structure, and magnetic fields of Jupiter and Saturn, we can begin to unravel their history. A comprehensive theory of giant planet evolution is necessary to answer the questions about planet formation that still perplex us, and it will be built on our understanding of these two gas giants.


The rapidly growing field of planetary science, buoyed by the unprecedented surge in exoplanet discoveries, calls for ever more sophisticated tools to understand the complex processes governing planetary evolution. To interpret the observational data and unravel the intriguing mysteries of these distant worlds, it is essential to delve into the intricate interplay of physical, chemical, and geological processes that shape planets over billions of years. Computational modeling plays a vital role in this endeavor, providing us with a virtual laboratory to study these complex phenomena.

We present the development of a new computational tool, named 'APPLE', designed to advance our modeling capabilities for planetary evolution. APPLE is a comprehensive, flexible, and robust code that integrates a diverse range of physical processes, from core formation and mantle convection to atmospheric dynamics and radiative heat transfer. The code enables us to model planets' life cycles, from the earliest stages of their existence to their eventual cooling, using state-of-the-art numerical methods.

Existing tools have made significant contributions to our understanding of planetary evolution, but many have limitations, including the isolated treatment of different planetary processes or simplifications in the underlying physics. Our new code, APPLE, addresses these limitations by providing a platform that holistically integrates the complex mechanisms that drive planetary evolution.

The primary goal of this paper is to present a detailed description of the APPLE code. We elucidate its structure, the numerical techniques employed, and the underlying physical principles. The versatility of APPLE is showcased through a series of test cases, illustrating its application across a wide range of planetary conditions and scenarios. This powerful new tool is poised to revolutionize our understanding of planetary evolution and will hopefully inspire and facilitate future research in planetary science.


what people have learned. Ideas coming from missions, in that spirit apple have been constructed. 

Space missions have introduced 
Juno stabily starified regions

